Market Segmentation Trees

We seek to provide an interpretable framework for segmenting users in a population for personalized decision-making. We propose a general methodology, Market Segmentation Trees (MSTs), for learning market segmentations explicitly driven by identifying differences in user response patterns. To demonstrate the versatility of our methodology, we design two new, specialized MST algorithms: (i) Choice Model Trees (CMTs), which can be used to predict a user's choice amongst multiple options and (ii) Isotonic Regression Trees (IRTs), which can be used to solve the bid landscape forecasting problem. We provide a theoretical analysis of the asymptotic running times of our algorithmic methods, which validates their computational tractability on large datasets. We also provide a customizable, open-source code base for training MSTs in Python which employs several strategies for scalability, including parallel processing and warm starts. Finally, we assess the practical performance of MSTs on several synthetic and real world datasets, showing that our method reliably finds market segmentations which accurately model response behavior.

==> ResponseLetter.tex <==
\begin{center}
\vspace{-20pt}
{\bf \large 
Response to the Review Team} \\ 
\vspace{16pt}

{\bf \large
Market Segmentation Trees (MSOM-20-025.R1)
}
\\

\vspace{16pt} 
%\today
\end{center}

 

\section*{Comments from Editor-in-Chief (serving as Department Editor)}

 

\textit{``Dear Author (this is to ensure anonymity): I have received 2 reviews and an Associate Editor (AE) report on your paper. (See below for instructions on how to view the reports.)   I thank the entire review team for their informative and constructive feedback. The entire team finds your revised version a big improvement.  Reviewer 1 recommended acceptance, and reviewer 2 has specific suggestions for you to improve the "interpretability" issue.  The AE agrees with reviewers and suggest you to dig in deeper on the interpretability aspect especially of the segments. I have reviewed all reports and find that reviewer 2's suggestion can be useful for you to improve the paper further.  As such, I would like to encourage you to follow the AE's suggestion to dig deeper on the interpretability issue. With some extra work, we hope your paper is likely to be accepted in the next round. Thank you, Chris Tang.
''}

 
 

\section*{Comments from Associate Editor}

 

\textit{``The revised version of the paper has improved a lot. The authors have done a great job revising the paper and addressing the comments from the review team. The new SwissMetro data set has also helped improve the case of the paper a lot. There are some additional minor comments the authors need to address. For this reason I recommend minor revision. In particular, I would like to ask the authors to dig in deeper on the interpretability aspect especially of the segments. One of the reviewers also provides more comments. This is particular important for the paper. Please also check for typos throughout the paper.''}

 
  

\section*{Comments from Referee 1}

 

\textit{``In this revision, the authors have put in a significant effort to address all of the reviewer comments from the previous round, and make an already strong paper even stronger. In particular, the new experiment with the SwissMetro data set is excellent, and the across-the-board improvement over a very diverse collection of benchmark models really makes a very compelling case for the method. I also enjoyed reading the new, more streamlined theoretical results and the accompanying proofs. I am happy to recommend that the paper be accepted. I only ask that the authors proofread the paper one more time before submitting their final files, just to catch any lingering typos or opportunities for better clarification (although I will admit that I did not spot any such cases on this second read). Congratulations to the authors on a very nice contribution to the literature!''}
 


\section*{Comments from Referee 2}

 
\textit{``I would like to first thank the reviewers for revising the manuscript. The updated paper is much more streamlined, and the authors have worked hard to incorporate all the comments that I made in the previous round. I do not have many comments. My only major comment is around interpretability. The authors have now added a section on interpretability to compare different algorithms. They present Figure 6, which presents MSE/AUC curves of the benchmark algorithms. While these demonstrate that the market segments have good predictive power, one interesting question is whether the market segments themselves are interpretable. In particular, the authors claim that one important outcome of the MSTs is the market segments that are generated. To show that the market segments are indeed intuitive, the authors can show different segments that are generated as a function of the input features (x). Then, the authors can compare the different outcome functions of each segment to show interesting insights on how the different segments differ from one another not just in terms of input features, but also in terms of outcomes. I am recommending a minor revision and look forward to reading the updated manuscript of the paper.''}
 

\bigskip

\textbf{A:} We thank the review team for their very positive and thoughtful feedback. Your comments throughout this process have greatly improved our paper and its potential impact. In this revision, we focused on leveraging the interpretability of our framework to illustrate how to extract insights / intuition from the trees constructed for both the CMT and IRT case studies. For your convenience, we have extracted the new additions to the paper and put them below so you can easily see them.

\underline{CMTs for Swissmetro Case Study}

{\color{blue}To gain intuition as to how utility model parameters differ across market segments, one can compare the values of option-specific parameters $\beta_{l,h}$ across different market segments $l$ and for each option $h$. To illustrate, Figure \ref{fig:betasS10_rr} provides a scatter plot showing each market segment's betas for Swissmetro's cost and travel time. As expected, nearly all of these betas are negative, implying that people prefer the Swissmetro option to have a shorter travel time and lower cost.
As an example of comparing betas across market segments, consider segments 1 and 2, which together represent the subset of people who are current rail users and travel for business; for this subset of people, we find that young people (market segment 1: age $\leq$ 24) are relatively more sensitive to cost and less sensitive to travel time than middle-aged people (market segment 2: 25 $\leq$ age $\leq$ 65).}

\begin{figure}[h]
    \centering
	\includegraphics[width=10cm]{Management_Science/beta_plot.png}
	\caption{{\color{blue}Scatter plot of betas for Swissmetro's cost and travel time, with each dot representing a pair of betas for its labeled market segment produced by the CMT with depth 4 for split S10.}}
	\label{fig:betasS10_rr}
\end{figure}

\underline{IRTs for DSP Case Study}

{\color{blue}In Section \ref{sec:DSP} and Appendix \ref{sec:DSPExp}, we observe across all 3 ad exchanges that IRTs using only 10 market segments perform better than IRKM models using up to 1000 market segments. A key advantage of these concise IRTs is their interpretability, as their splits can be easily examined to determine which features have the greatest importance in customizing bids and predicting ad auction outcomes. To demonstrate this, Figure \ref{fig:irtsplits} visualizes the leaf models resulting from two different terminal splits found within the 10-segment IRTs trained on ad exchanges 1 and 2. Figure \ref{fig:channelsplit} corresponds to a terminal split on \textit{ad display channel} which assesses whether the display of the ad spot corresponds to desktop or mobile. The figure indicates that mobile display ads typically receive higher bids than desktop display ads, which could be due to mobile ads often having a higher click-through-rate (CTR) than desktop ads for this ad exchange. Figure \ref{fig:aspectratiosplit} visualizes the bid landscapes resulting from splitting on the value of the \textit{aspect ratio} of the ad spot (defined as the ratio of the width to the height of the ad spot). The figure suggests that aspect ratios greater than 3.5 typically receive lower bids than aspect ratios less than 3.5. This finding may be partially driven by aspect ratios greater than 3.5 also having predominately desktop displays - often with a lower CTR - as opposed to mobile displays (96\% have desktop displays for aspect ratios greater than 3.5 vs. 68\% for smaller aspect ratios). %However, there is likely another reason linking high aspect ratios to less competitive ad auctions, because the IRT could have instead split on the ad display channel feature if it was the sole driver behind the bid landscape discrepancies. 
While IRTs can be used to study predictive links between features and response model differences (thereby aiding personalization), it is important to note that IRTs alone cannot be used to determine \textit{causal} relationships between features and differences in response models.}

\begin{figure}[h]
\FIGURE
  {
	\centering
	\begin{subfigure}{.45\linewidth}
		\centering
		\includegraphics[width=0.92\linewidth]{ExchID2_ChannelTypeSplit_paper}
		\caption{\small IR models from channel split}
		\vspace{0.1cm}
		\label{fig:channelsplit_rr}
	\end{subfigure}%
	\begin{subfigure}{.45\linewidth}
		\centering
		\includegraphics[width=0.92\linewidth]{ExchID1_AspectRatioSplit_paper}
		\caption{\small IR models from aspect ratio split}
		\vspace{0.1cm}
		\label{fig:aspectratiosplit_rr}
	\end{subfigure}
	}
{{\color{blue}Estimated bid landscapes from splits in the trained IRTs from Section \ref{sec:DSP}}. \label{fig:irtsplits_rr}}
{{\color{blue}Figure \ref{fig:channelsplit_rr} is from an IRT pruned to 10 leaves trained on bidding data from Exchange 2. Figure \ref{fig:aspectratiosplit_rr} is from an IRT pruned to 10 leaves trained on bidding data from Exchange 1.}}
\end{figure}

==> counterexample.tex <==

\section{Suboptimality of Customer Valuation Splitting}

\subsection{Background}

Note: in the following discussion, we will focus on the application of personalized pricing of a single product. However, these results are of practical relevance to any price-setting applications (e.g., bid pricing).

Assume that customer purchasing behavior can be characterized by $M$ distinct customer ``types'', each with their own valuation distribution for the product. A new customer is sampled from the $i$th type with probability $\alpha_i$, where $\alpha_1+...+\alpha_M = 1$. We assume that it is possible to perfectly classify arriving customers into their respective types on the basis of available feature information, such as the age and prior purchase history of the customer. Our goal is to explore new algorithms for market segmentation which learn the true mapping of features to customer types from data.

Let $V_i$ denote the random valuation of a customer from segment $i$. A simple approach to market segmentation might be to assume that the expected customer valuations in each segment are distinct, i.e. $E[V_i] \neq E[V_j]$ for all $i \neq j$. One could then apply a standard machine-learning algorithm, such as CART regression trees, to partition the feature space into segments with different expected customer valuations. However, we argue that for the purposes of revenue maximization, it is important to consider the \textit{full distribution} of $V_i$ when performing market segmentation, as two segments with the same $E[V_i]$ can have very different optimal pricing strategies.

In the next section, we show that the revenue from segmenting on the full valuation distribution can be $M$ times as large as the revenue attained from segmenting on expected customer valuations alone.

\subsection{Theorem and Proof}

As in the previous section, let $M$ denote the number of customer segments, or customer ``types''. Let $\mathcal{F}_{V_i}$ denote the distribution of the valuation $V_i$ in segment $i$. We assume that customers are perfectly separable into their respective types through use of their features. Thus, by performing market segmentation on the basis of valuation distributions $\mathcal{F}_{V_i}$, it is possible to correctly classify the type of a new customer and assign her a personalized price $p$ for the product. Denote the optimal expected revenue from personalizing prices in the $M$ segments by ``OERS'' -- the Optimal Expected Revenue with Segmentation.

We will constrain the valuation distributions so that the expected customer valuations in all segments are equal, i.e. $E[V_i] = E[V_j]$ for all $i \neq j$. Then, a market segmentation procedure on the basis of expected customer valuations would fail to capture any of the $M$ true segments. In this case, price personalization is not possible, and a single price is thus assigned to all customers. Denote the best possible revenue from this procedure by ``OERNS'' -- the Optimal Expected Revenue with No Segmentation.

As in the previous section, let ``mixing parameter'' $\alpha_i$ denote the probability that a new customer is sampled from segment $i$. We will now prove the following theorem, which demonstrates the potential for significant revenue loss from segmenting customers on the basis of expected valuations alone:

\begin{thm}  \label{thm:bound}
Fix the number of segments $M$. For any $\epsilon > 0$, there exists valuation distributions $\mathcal{F}_{V_1},...,\mathcal{F}_{V_M}$ and mixing parameters $\alpha_1,...,\alpha_M$ such that

\begin{equation}\label{eqn:theoremeq1}
    \frac{OERS}{OERNS} \geq \frac{M}{1+\epsilon} \, .
\end{equation} 

Furthermore, for any set of $M$ valuation distributions and mixing parameters,

\begin{equation}\label{eqn:theoremeq2}
    \frac{OERS}{OERNS} \leq M \, ,
\end{equation} 



\noindent
thus the bound (\ref{eqn:theoremeq1}) is tight to within a factor of $(1+\epsilon)$.
\end{thm}

\textit{Proof:} To demonstrate the practical relevance of Theorem \ref{thm:bound}, we will prove the theorem for two different families of valuation distributions:

\begin{enumerate}
    \item \textbf{Two-point Distribution}. $V_i$ is discrete, with:
    
    \begin{equation*}
  V_i=\begin{cases}
    v_i, & \text{with probability} \,\,\, q_i.\\
    0, & \text{otherwise}.
  \end{cases}
\end{equation*}

    \item \textbf{Logistic Distribution}: $V_i \sim Logistic(\mu_i, s_i)$, i.e.
    
    \begin{equation*}
   P(V_i \leq v) = \frac{1}{1+e^-\frac{v-\mu_i}{s_i}}
\end{equation*}

\end{enumerate}

\noindent Further, we will provide a lemma which offers a general framework for proving the theorem under other valuation distribution families.

We first define some notation. Note that a customer will purchase a product at price $p$ if and only if his valuation is greater than $p$. Let $R_i(p) = E[p \mathbb{I}\{V_i \geq p\}] = p P(V_i \geq p)$ denote the expected revenue from charging price $p$ to a customer from segment $i$. Let $p_i^* = \arg\max_{p \geq 0} R_i(p)$ be the optimal personalized price from segment $i$, and let $R_i^* = R_i(p_i^*)$ be the corresponding optimal expected revenue. Without loss of generality, we assume that $R_i^* > 0$ for all $i$.

We now proceed with proving statement (\ref{eqn:theoremeq2}) of the theorem. The optimal expected revenue from personalized pricing, OERS, is simply:

\begin{equation*} 
    OERS = \alpha_1 R_1^* + ... + \alpha_M R_M^*
\end{equation*}

Let $k = \arg \max_{1 \leq i \leq M} \alpha_i R_i^*$. Then, $OERS \leq M \alpha_k R_k^*.$ If we were to charge price $p =  p_k^*$ to all customers, then the expected revenue would be at least $\alpha_k R_k^*$ from the customers sampled from segment $k$. Thus, $OERNS \geq \alpha_k R_k^*$, and

\begin{equation*}
    \frac{OERS}{OERNS} \leq \frac{M \alpha_k R_k^*}{\alpha_k R_k^*} = M \, .
\end{equation*}

This proves statement (\ref{eqn:theoremeq2}). We now proceed with proving (\ref{eqn:theoremeq1}). With respect to any set of valuation distributions, we will henceforth index the segments so that their optimal prices are in increasing order: $p_1^* \leq p_2^* \leq ... \leq p_M^*$. Define the \textit{partition points} $\{ \rho_i \}_{0 \leq i \leq M}$ to be a collection of points which partition $[0,\infty)$ in the following way:

\begin{eqnarray*}
\begin{cases}
    \rho_0 = 0 \\
    \rho_M = \infty \\
    \rho_{i-1} \leq p_i^*  \leq \rho_{i}, \,\,\, \text{for} \,\,\, i \in \{1,...,M\}
\end{cases}
\end{eqnarray*}


We will use the following lemma in proving the theorem. The proof of the lemma can be found in the appendix.

\begin{lem}
For a fixed $\delta > 0$, assume there exists valuation distributions $\mathcal{F}_{V_1},...,\mathcal{F}_{V_M}$ and mixing parameters $\alpha_1,...,\alpha_M$ which satisfy the following conditions:

\begin{enumerate}
    \item $\alpha_i R_i^* = \alpha_j R_j^*$ for all $i \neq j$.
    \item There exists partition points $\{ \rho_i \}_{0 \leq i \leq M}$ such that, for all $i \neq j$,
    \begin{equation*}
        \max_{\rho_{i-1} \leq p  \leq \rho_{i}}\frac{R_j(p)}{R_j^*} \leq \delta \, .
    \end{equation*}
\end{enumerate}

Then, under $\mathcal{F}_{V_1},...,\mathcal{F}_{V_M}$ and $\alpha_1,...,\alpha_M$,

\begin{equation*}
    \frac{OERS}{OERNS} \geq \frac{M}{1+\delta (M-1)} \, .
\end{equation*} 

\end{lem}

The first lemma condition states that the optimal expected revenues from personalized pricing in any segment, weighted by the mixing parameters, must be equal in all segments. If this were not the case, then we could achieve a revenue strictly greater than $OERS/M$ by simply charging price $p =  p_k^*$ to all customers, where $k = \arg \max_{1 \leq i \leq M} \alpha_i R_i^*$. The second condition states that prices which attain high revenues for customers from segment $i$ yield almost no revenue with respect to any other segment $j$. Thus, the revenue distributions for each segment yield completely different optimal prices, and by charging a single price to all customers, we can only profit from one particular customer segment. This leads to $OERNS$ being roughly $1/M$th the revenue of $OERS$.

To prove the theorem, we will construct valuation distributions $\mathcal{F}_{V_1},...,\mathcal{F}_{V_M}$ and mixing parameters $\alpha_1,...,\alpha_M$ which satisfy the conditions of the lemma for \textit{any} $\delta > 0$. We will do so for two valuation distribution families -- the two-point distribution and the logistic distribution.

\subsubsection{Two-Point Distribution}

In this section, we consider a very simple discrete model for the valuations $V_i$:
    
    \begin{equation*}
  V_i=\begin{cases}
    v_i, & \text{with probability} \,\,\, q_i.\\
    0, & \text{otherwise}.
  \end{cases}
\end{equation*}

\noindent For each segment $i$, $1 \leq i \leq M$, set

\begin{eqnarray*}
v_i &=& N^i \\
q_i &=& \frac{1}{N^i} \\
\alpha_i &=& \frac{1}{M}
\end{eqnarray*}

\noindent where the definitions of $v_i$ and $q_i$ depend on a positive constant, $N$. First, note that the expected valuations in all segments are equal: $E[V_i] = v_i q_i = 1$. The expected revenue from charging price $p$ to a customer from segment $i$ is:

\begin{eqnarray*}
    R_i(p) &=& \begin{cases}
    p \, q_i, & p \leq v_i \\
    0, & \text{otherwise} .
  \end{cases} \\
  &=& \begin{cases}
    p/N^i, & p \leq N^i \\
    0, & \text{otherwise} .
  \end{cases}
\end{eqnarray*}

The revenue-maximizing price is attained at $p_i^* = N^i$, with a corresponding expected revenue of $R_i^* = R_i(N^i) = 1$. Condition 1 of the lemma is thus satisfied for all values of $N$, with $\alpha_i R_i^* = 1/M$. We now focus on condition 2. Define the partition points $\{ \rho_i \}_{0 \leq i \leq M}$ in the following way:

\begin{eqnarray*}
\begin{cases}
    \rho_0 = 0 \\
    \rho_M = \infty \\
    \rho_{i} = \sqrt{p_i^* p_{i+1}^*} = N^i \sqrt{N}, \,\,\, \text{for} \,\,\, i \in \{1,...,M-1\}
\end{cases}
\end{eqnarray*}  

\noindent Note that $\rho_{i}$ satisfies $\rho_{i-1} \leq p_i^*  \leq \rho_{i}$ for all $i$. We will show the following statement holds for all $i \neq j$:

    \begin{equation} \label{eqn:cond2}
        \lim_{N \rightarrow \infty} \max_{\rho_{i-1} \leq p  \leq \rho_{i}}\frac{R_j(p)}{R_j^*} = 0 \, .
    \end{equation}

\noindent The above equality implies that there exist valuation distributions which satisfy lemma condition 2 for all $\delta > 0$, which proves the theorem. Note that:

\begin{eqnarray*}
    \max_{\rho_{i-1} \leq p  \leq \rho_{i}} R_j(p) &=& \begin{cases}
    0, & j \leq i - 1 \\
    R_j(\rho_{i}), & j \geq i + 1 
  \end{cases} \\
  &=& \begin{cases}
    0, & j \leq i - 1 \\
    N^i \sqrt{N}/N^j, & j \geq i + 1 .
  \end{cases}
\end{eqnarray*}

\noindent Given that $R_j^* = 1$ for all $i$, (\ref{eqn:cond2}) clearly holds, as  $\lim_{N \rightarrow \infty} N^i \sqrt{N}/N^j = 0$ for $j \geq i + 1$.

\subsubsection{Logistic Distribution}

Although the two-point valuation distributions from the previous section satisfy the conditions of Theorem 1, such distributions are seldom used in practice to model customer valuations. We now consider using a more practically-relevant distribution -- the logistic distribution -- to model customer valuations. Assume that $V_i \sim Logistic(\mu_i, s_i)$, with
    
\begin{equation*}
   P(V_i \leq v) = \frac{1}{1+e^-\frac{v-\mu_i}{s_i}}
\end{equation*}

For each segment $i$, set:

\begin{eqnarray*}
\mu_i &=& \mu \\
s_i &=& N^i
\end{eqnarray*}

\noindent where $\mu$ is an arbitrary constant. As in the previous section, we will eventually use a limiting argument on $N$ to prove the theorem. Since $E[V_i] = \mu_i = \mu$, the expected valuations in all segments are equal by design. The expected revenue function in segment $i$ is:

\begin{eqnarray*}
    R_i(p) &=& p P(V_i \geq p) \\
    &=& \frac{p}{1+e^\frac{p-\mu}{N^i}}
\end{eqnarray*}

Let $K_i := W(e^{N^{-i}\mu - 1})$, where $W(\cdot)$ is the Lambert-W function. Then, the price which maximizes $R_i(p)$ is given by $p_i^* = (K_i + 1) N^i$, with a corresponding revenue of $R_i^* = K_i N^i$. Define the mixing parameters for all segments $i$ as follows:

\begin{equation*}
    \alpha_i = \frac{K_i^{-1} N^{-i}}{\sum_{j=1}^M K_j^{-1} N^{-j}}
\end{equation*}

Then, lemma condition 1 is satisfied for all $\mu$ and $N$: 

\begin{equation*}
    \alpha_i R_i^* = \frac{1}{\sum_{j=1}^M K_j^{-1} N^{-j}} \, .
\end{equation*}

We thus turn our attention to condition 2. As in the previous section, we will define the partition points $\{ \rho_i \}_{0 \leq i \leq M}$ using the geometric mean between two sequential optimal segment prices:

\begin{eqnarray*}
\begin{cases}
    \rho_0 = 0 \\
    \rho_M = \infty \\
    \rho_{i} = \sqrt{p_i^* p_{i+1}^*} = \sqrt{K_i + 1} \sqrt{K_{i+1} + 1} N^i \sqrt{N}, \,\,\, \text{for} \,\,\, i \in \{1,...,M-1\}
\end{cases}
\end{eqnarray*}  

\noindent Note that $\rho_{i}$ satisfies $\rho_{i-1} \leq p_i^*  \leq \rho_{i}$ for all $i$. Following the procedure in the previous section, it is sufficient to show that for all $i \neq j$:

    \begin{equation*}
        \lim_{N \rightarrow \infty} \max_{\rho_{i-1} \leq p  \leq \rho_{i}}\frac{R_j(p)}{R_j^*} = 0 \, .
    \end{equation*}

Fix $i \neq j$. We will first consider the case of $i \neq M$:

\begin{eqnarray*}
&& \max_{\rho_{i-1} \leq p  \leq \rho_{i}}\frac{R_j(p)}{R_j^*} \\
&=& \max_{\rho_{i-1} \leq p  \leq \rho_{i}}\frac{p}{R_j^*} P(V_j \geq p) \\
&\leq& \begin{cases}
\dfrac{\rho_{i}}{R_j^*}P(V_j \geq \rho_{i-1}), & j \leq i - 1, \,\,\, i \neq M \\ \dfrac{\rho_{i}}{R_j^*}, & j \geq i + 1, \,\,\, i \neq M
\end{cases} \\
&=& \begin{cases}
\dfrac{\sqrt{K_i + 1} \sqrt{K_{i+1} + 1} N^i \sqrt{N}}{K_j N^j}\dfrac{1}{1+\exp\{\frac{\sqrt{K_{i-1} + 1} \sqrt{K_{i} + 1} N^{i-1} \sqrt{N} - \mu}{N^j}\}}, & j \leq i - 1, \,\,\, i \neq M \\ \dfrac{\sqrt{K_i + 1} \sqrt{K_{i+1} + 1} N^i \sqrt{N}}{K_j N^j}, & j \geq i + 1, \,\,\, i \neq M
\end{cases} \\
\end{eqnarray*}

Note that $\lim_{N \rightarrow \infty} K_i = W(e^{-1}) \approx 0.28$ for all $i$. Thus, one can easily verify that the quantities in the above expression approach zero as $N \rightarrow \infty$. We now consider $i = M$. For $j \neq i$, i.e. $j \leq M - 1$, the log-concavity of $R_j(p)$ implies that $R_j(p_j^*) \geq R_j(p_M^*) \geq R_j(p)$ for $p \geq p_M^*$. Thus, for $j \leq M - 1$,

\begin{eqnarray*}
&& \max_{\rho_{M-1} \leq p  \leq \rho_{M}}\frac{R_j(p)}{R_j^*} \\
&=& \max_{\rho_{M-1} \leq p  \leq p_M^*}\frac{R_j(p)}{R_j^*}\\
&=& \max_{\rho_{M-1} \leq p  \leq p_M^*} \frac{p}{R_j^*} P(V_j \geq p) \\
&\leq& \frac{p_M^*}{R_j^*} P(V_j \geq \rho_{M-1}) \\
&=& \frac{(K_M + 1) N^M}{K_j N^j} \dfrac{1}{1+\exp\{\frac{\sqrt{K_{M-1} + 1} \sqrt{K_{M} + 1} N^{M-1} \sqrt{N} - \mu}{N^j}\}} \, ,
\end{eqnarray*}

\noindent and the above quantity approaches zero as $N \rightarrow \infty$. This concludes the proof. \hfill $\blacksquare$

\section{Proof of Lemma \ref{repeatlemma}}

Here we will prove Lemma \ref{repeatlemma}, which is restated below:

\setcounter{lemma}{0}

\begin{lem} \label{repeatlemma}
For a fixed $\delta > 0$, assume that the valuation distributions $\mathcal{F}_{V_1},...,\mathcal{F}_{V_M}$ and mixing parameters $\alpha_1,...,\alpha_M$ satisfy the following conditions:

\begin{enumerate}
    \item $\alpha_i R_i^* = \alpha_j R_j^*$ for all $i \neq j$.
    \item There exists partition points $\{ \rho_i \}_{0 \leq i \leq M}$ such that, for all $i \neq j$,
    \begin{equation*}
        \max_{\rho_{i-1} \leq p  \leq \rho_{i}}\frac{R_j(p)}{R_j^*} \leq \delta \, .
    \end{equation*}
\end{enumerate}

Then,

\begin{equation*}
    \frac{OERS}{OERNS} \geq \frac{M}{1+\delta (M-1)} \, .
\end{equation*} 

\end{lem}

\textit{Proof:} First, note that condition 1 together with the equation $\alpha_1+...+\alpha_M = 1$ yields a unique solution for the mixing parameters:

\begin{equation*}
    \alpha_i = \frac{R_i^{*-1}}{\sum_j R_j^{*-1}} \,\,\, \text{for all} \,\,\, i \, .
\end{equation*}

Thus, the optimal revenue with segmentation is as follows:

\begin{equation*}
    OERS = \alpha_1 R_1^* + ... + \alpha_M R_M^* = \frac{M}{\sum_j R_j^{*-1}} \, .
\end{equation*}

Also, $OERNS$ can be easily bounded using condition 2:

\begin{eqnarray*}
    OERNS &=& \max_{p \geq 0} \sum_{j=1}^M \alpha_j R_j(p) \\
    &=& \max_{1 \leq i \leq M} \max_{\rho_{i-1} \leq p  \leq \rho_{i}} \sum_{j=1}^M \alpha_j R_j(p) \\
    &=& \frac{1}{\sum_j R_j^{*-1}} \max_{1 \leq i \leq M} \max_{\rho_{i-1} \leq p  \leq \rho_{i}} \sum_{j=1}^M  \frac{R_j(p)}{R_j^*} \\
    &\leq& \frac{1}{\sum_j R_j^{*-1}} \max_{1 \leq i \leq M} \max_{\rho_{i-1} \leq p  \leq \rho_{i}} \frac{R_i(p)}{R_i^*} + \delta (M-1) \\
    &=& \frac{1}{\sum_j R_j^{*-1}} \max_{1 \leq i \leq M} \frac{R_i(p_i^*)}{R_i^*} + \delta (M-1) \\
    &=& \frac{1+\delta (M-1)}{\sum_j R_j^{*-1}}
\end{eqnarray*}

Therefore, 

\begin{equation*}
    \frac{OERS}{OERNS} \geq \frac{M}{1+\delta (M-1)} \, ,
\end{equation*} 

\noindent which concludes the proof of the lemma. \hfill $\blacksquare$
